SparsyFed: Sparse Adaptive Federated Training

Sparse training is often adopted in cross-device federated learning (FL) environments where constrained devices collaboratively train a machine learning model on private data by exchanging pseudo-gradients across heterogeneous networks. Although sparse training methods can reduce communication overhead and computational burden in FL, they are often not used in practice for the following key reasons: (1) data heterogeneity makes it harder for clients to reach consensus on sparse models compared to dense ones, requiring longer training; (2) methods for obtaining sparse masks lack adaptivity to accommodate very heterogeneous data distributions, crucial in cross-device FL; and (3) additional hyperparameters are required, which are notably challenging to tune in FL. This paper presents SparsyFed, a practical federated sparse training method that critically addresses the problems above. Previous works have only solved one or two of these challenges at the expense of introducing new trade-offs, such as clients' consensus on masks versus sparsity pattern adaptivity. We show that SparsyFed simultaneously (1) can produce 95% sparse models, with negligible degradation in accuracy, while only needing a single hyperparameter, (2) achieves a per-round weight regrowth 200 times smaller than previous methods, and (3) allows the sparse masks to adapt to highly heterogeneous data distributions and outperform all baselines under such conditions.

==> authors.tex <==
\let\hypersetup\truehypersetup
\makeatletter
\newcommand{\myfnsymbol}[1]{%
  \expandafter\@myfnsymbol\csname c@#1\endcsname
}
% Mapping of how the \thanks symbols will be interpreted sequentially
\newcommand{\@myfnsymbol}[1]{%
  \ifcase #1
    % 0
  \or 1% 1
  \or 2% 2
  \or 3% 2
  \or \TextOrMath{\textasteriskcentered}{*}% 3
  \or \TextOrMath{\textasteriskcentered}{*}\TextOrMath{\textasteriskcentered}{*}% 4
  \or \TextOrMath{\textdagger}{\dagger}% 5
  \or \TextOrMath{\textasteriskcentered}{*},\TextOrMath{\textasteriskcentered}{*}\TextOrMath{\textasteriskcentered}{*}% 6
  \fi
}
% Just to make things explicit in the code what it means
\newcommand{\affiliationA}{\@myfnsymbol{1}}
\newcommand{\affiliationB}{\@myfnsymbol{2}}
\newcommand{\affiliationC}{\@myfnsymbol{3}}
\newcommand{\equalcontributor}{\@myfnsymbol{4}}
\newcommand{\biequalcontributor}{\@myfnsymbol{5}}
\newcommand{\correspondingA}{\@myfnsymbol{6}}


% Authors must not appear in the submitted version. They should be hidden
% as long as the \iclrfinalcopy macro remains commented out below.
% Non-anonymous submissions will be rejected without review.

\author{
Adriano Guastella\textsuperscript{\equalcontributor,\affiliationA}
\qquad\qquad\qquad
Lorenzo Sani\textsuperscript{\equalcontributor,\affiliationB,\affiliationC}
\qquad\qquad\qquad
Alex Iacob\textsuperscript{\affiliationB,\affiliationC}
\AND
~~Alessio Mora\textsuperscript{\affiliationA}
\qquad\qquad\qquad\qquad
Paolo Bellavista\textsuperscript{\affiliationA}
\qquad\qquad~~~
Nicholas D. Lane\textsuperscript{\affiliationB,\affiliationC}
}


% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to \LaTeX{} to determine where to break
% the lines. Using \AND forces a linebreak at that point. So, if \LaTeX{}
% puts 3 of 4 authors names on the first line, and the last on the second
% line, try using \AND instead of \And before the third author name.

==> tables/accuracy_all.tex <==


\begin{table}[!ht]
    \makebox[1 \textwidth][c]{       %centering table
    \resizebox{1.3 \textwidth}{!}{   %resize table
    \begin{tabular}{l *{13}{c}}
    \toprule
        \multirow{2}{*}{Dataset}
        & \multirow{2}{*}{Sparsity}
        & \multicolumn{3}{c}{Resnet18}
        & \multicolumn{3}{c}{ZeroFL}
        & \multicolumn{3}{c}{FLASH}
        & \multicolumn{3}{c}{\method} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
        & & $\alpha=10^3$ & $\alpha=1.0$ & $\alpha=0.1$ & $\alpha=10^3$ & $\alpha=1.0$ & $\alpha=0.1$ & $\alpha=10^3$ & $\alpha=1.0$ & $\alpha=0.1$ & $\alpha=10^3$ & $\alpha=1.0$ & $\alpha=0.1$ \\
    \midrule
        \multirow{6}{*}{CIFAR10} 
        & dense & 85.14 $\pm$ 1.18 & 83.70 $\pm$ 1.70 & 73.81 $\pm$ 4.84  & - & - & - & - & - & - & - & - & - \\
        & 0.9   & 82.16 $\pm$ 0.80 & 80.56 $\pm$ 1.90 & 69.79 $\pm$ 3.78  & 78.67 $\pm$ 1.52 & 76.16 $\pm$ 1.30 & 67.40 $\pm$ 4.11 & 82.57 $\pm$ 2.05  & 81.15 $\pm$ 1.03 & 71.87 $\pm$ 2.63 & 84.31 $\pm$ 0.86 & 82.13 $\pm$ 1.53 & 75.00 $\pm$ 2.78 \\
        & 0.95  & 77.92 $\pm$ 0.97 & 74.71 $\pm$ 3.29 & 60.00 $\pm$ 4.66  & 76.16 $\pm$ 1.28 & 75.53 $\pm$ 2.27 & 61.55 $\pm$ 4.18 & 82.22 $\pm$ 0.14  & 79.36 $\pm$ 1.03 & 72.08 $\pm$ 2.09 & 84.25 $\pm$ 1.38 & 82.60 $\pm$ 1.58 & 75.95 $\pm$ 3.39 \\
        & 0.99  & 68.11 $\pm$ 3.50 & 66.27 $\pm$ 5.08 & 43.96 $\pm$ 11.99 & 72.40 $\pm$ 1.08 & 70.71 $\pm$ 0.15 & 51.71 $\pm$ 3.54 & 77.48 $\pm$ 2.86  & 73.45 $\pm$ 1.37 & 56.91 $\pm$ 3.55 & 77.16 $\pm$ 0.85 & 77.71 $\pm$ 1.69 & 63.69 $\pm$ 3.90 \\
        & 0.995 & 54.49 $\pm$ 8.70 & 63.82 $\pm$ 2.41 & 19.02 $\pm$ 10.77 & 60.31 $\pm$ 4.11 & 56.02 $\pm$ 3.95 & 41.33 $\pm$ 3.64 & 71.85 $\pm$ 1.63  & 69.15 $\pm$ 1.60 & 52.15 $\pm$ 3.87 & 72.71 $\pm$ 0.65 & 70.01 $\pm$ 0.43 & 56.79 $\pm$ 3.97 \\
        & 0.999 & 17.87 $\pm$ 6.22 & 31.79 $\pm$ 19.10 & 11.50 $\pm$ 4.49 & 21.91 $\pm$ 1.11 & 17.66 $\pm$ 8.34 & 18.76 $\pm$ 4.28 & 46.43 $\pm$ 16.73 & 36.07 $\pm$ 7.49 & 29.31 $\pm$ 6.75 & 55.24 $\pm$ 2.09 & 51.39 $\pm$ 3.19 & 43.68 $\pm$ 7.61 \\
    \midrule
        \multirow{6}{*}{CIFAR100} 
        & dense & 53.79 $\pm$ 1.63  & 52.29 $\pm$ 1.14  & 48.34 $\pm$ 2.71  & - & - & - & - & - & - & - & - & - \\
        & 0.9   & 46.47 $\pm$ 1.74  & 46.57 $\pm$ 1.71  & 41.96 $\pm$ 2.16  & 44.11 $\pm$ 0.93 & 40.70 $\pm$ 4.72 & 31.92 $\pm$ 7.65 & 53.06 $\pm$ 1.10 & 51.99 $\pm$ 0.21 & 45.59 $\pm$ 0.75  & 54.44 $\pm$ 1.33 & 53.08 $\pm$ 0.90 & 48.37 $\pm$ 1.73 \\
        & 0.95  & 13.45 $\pm$ 21.45 & 28.07 $\pm$ 23.27 & 11.48 $\pm$ 17.51 & 33.67 $\pm$ 3.34 & 38.82 $\pm$ 1.75 & 34.21 $\pm$ 7.65 & 49.25 $\pm$ 1.63 & 47.19 $\pm$ 1.88 & 44.31 $\pm$ 2.14  & 54.33 $\pm$ 1.48 & 52.81 $\pm$ 1.72 & 48.27 $\pm$ 2.70 \\
        & 0.99  & 1.54 $\pm$ 1.22   & 19.65 $\pm$ 16.30 & 0.14 $\pm$ 0.72   & 10.59 $\pm$ 2.48 & 18.97 $\pm$ 2.08 & 13.07 $\pm$ 2.26 & 44.40 $\pm$ 1.77 & 42.76 $\pm$ 4.08 & 34.75 $\pm$ 3.38  & 47.62 $\pm$ 1.67 & 46.64 $\pm$ 1.59 & 41.03 $\pm$ 2.14 \\
        & 0.995 & 0.97 $\pm$ 0.64   & 9.51 $\pm$ 14.81  & 0.14 $\pm$ 0.72   & 4.04 $\pm$ 3.43  & 6.01 $\pm$ 4.74  & 7.04 $\pm$ 5.25  & 36.82 $\pm$ 1.72 & 36.43 $\pm$ 4.97 & 26.44 $\pm$ 17.35 & 42.05 $\pm$ 1.21 & 42.21 $\pm$ 1.03 & 35.72 $\pm$ 2.01 \\
        & 0.999 & 0.97 $\pm$ 0.64   & 3.81 $\pm$ 2.18   & 0.14 $\pm$ 0.72   & 0.87 $\pm$ 0.21  & 1.96 $\pm$ 0.66  & 1.66 $\pm$ 0.97  & 9.61 $\pm$ 3.61  & 5.80 $\pm$ 2.86  & 3.56 $\pm$ 2.07   & 13.85 $\pm$ 1.01 & 15.96 $\pm$ 0.64 & 13.84 $\pm$ 3.69 \\
    \midrule
        & dense  & 92.98 $\pm$ 0.67 & 91.49 $\pm$ 0.94  & 80.15 $\pm$ 2.69 & - & - & - & - & - & - & - & - & - \\
        & 0.9    & 85.53 $\pm$ 0.84 & 84.28 $\pm$ 0.88  & 65.44 $\pm$ 0.97 & 89.12 $\pm$ 1.11 & 87.79 $\pm$ 1.40 & 77.15 $\pm$ 1.77 & 89.89 $\pm$ 0.74 & 88.68 $\pm$ 1.72 & 77.15 $\pm$ 0.77 & 91.34 $\pm$ 0.52 & 92.32 $\pm$ 1.59 & 79.67 $\pm$ 2.78 \\
Speech  & 0.95   & 80.19 $\pm$ 1.92 & 78.58 $\pm$ 0.44  & 57.39 $\pm$ 1.04 & 85.63 $\pm$ 1.12 & 84.29 $\pm$ 1.50 & 71.28 $\pm$ 2.75 & 88.16 $\pm$ 1.37 & 84.89 $\pm$ 0.49 & 71.28 $\pm$ 1.75 & 89.79 $\pm$ 0.21 & 89.14 $\pm$ 1.15 & 75.46 $\pm$ 2.24 \\
Commands& 0.99   & 67.67 $\pm$ 2.32 & 65.01 $\pm$ 0.84  & 50.42 $\pm$ 6.26 & 60.79 $\pm$ 2.44 & 57.79 $\pm$ 0.82 & 53.55 $\pm$ 4.00 & 76.41 $\pm$ 1.31 & 69.22 $\pm$ 1.59 & 53.55 $\pm$ 2.00 & 77.00 $\pm$ 0.73 & 75.82 $\pm$ 3.72 & 56.69 $\pm$ 4.56 \\
        & 0.995  & 63.63 $\pm$ 3.24 & 56.73 $\pm$ 1.00  & 34.20 $\pm$ 1.43 & 41.16 $\pm$ 3.10 & 37.16 $\pm$ 2.71 & 43.16 $\pm$ 3.47 & 67.54 $\pm$ 1.15 & 58.23 $\pm$ 1.84 & 43.16 $\pm$ 3.47 & 70.03 $\pm$ 1.14 & 68.02 $\pm$ 3.14 & 48.30 $\pm$ 5.39 \\
        & 0.999  & 19.75 $\pm$ 1.73 & 21.56 $\pm$ 12.79 & 19.25 $\pm$ 6.01 & 16.77 $\pm$ 6.23 & 10.10 $\pm$ 4.01 & 17.14 $\pm$ 2.97 & 31.83 $\pm$ 2.18 & 17.70 $\pm$ 2.58 & 17.14 $\pm$ 2.97 & 49.27 $\pm$ 0.50 & 47.43 $\pm$ 1.66 & 29.24 $\pm$ 2.34 \\
    \bottomrule
    \end{tabular}
    }}
    \caption{Aggregated results for CIFAR10, CIFAR100, and Google Speech Command datasets, with Resnet18, ZeroFL, FLASH, and SparsyFed implementations.}
\end{table}

==> tables/naive_powerpropagatio.tex <==
\begin{table}[!ht]
    \centering
    \label{tab:naive_powerprop}
    \begin{tabular}{@{}lccc@{}}
    \toprule
    \multirow{2}{*}{Sparsity} & \multicolumn{3}{c}{Naive Powerpropagation} \\
    \cmidrule(lr){2-4}
    & $\alpha=10^3$ (IID) & $\alpha=1.0$ (non-IID) & $\alpha=0.1$ (non-IID) \\
    \midrule
    0.000   & 84.69 $\pm$ 1.57 & 84.31 $\pm$ 1.01 & 74.86 $\pm$ 2.28 \\
    0.900   & 71.41 $\pm$ 7.01 & 66.70 $\pm$ 3.76 & 45.82 $\pm$ 6.31 \\
    0.950   & 35.02 $\pm$ 6.37 & 33.84 $\pm$ 13.71 & 24.28 $\pm$ 8.79 \\
    0.990   & 12.49 $\pm$ 4.17 & 12.30 $\pm$ 3.68 & 9.28 $\pm$ 2.52 \\
    0.995   & 10.33 $\pm$ 0.57 & 10.03 $\pm$ 0.05 & 9.74 $\pm$ 3.24 \\
    0.999   & 9.86 $\pm$ 0.25 & 10.01 $\pm$ 0.02 & 11.67 $\pm$ 6.66 \\
    \bottomrule
    \end{tabular}
    \caption{Accuracy comparison for Naive Powerpropagation on CIFAR-10 with different LDA settings ($\alpha=10^3$, $\alpha=1.0$, and $\alpha=0.1$).}
\end{table}
